A User-Study Protocol for Evaluation of Formal Verification Results and their Explanation

Context: The complexity of modern safety-critical systems in industries keep on increasing due to the rising number of features and functionalities. This calls for formal methods in order to entrust confidence in such systems. Nevertheless, using formal methods in industry is demanding because of usability issues, e.g., the difficulty of understanding model checking results. Thus the hypothesis is, presenting the result of model checker results in a user-friendly manner could promote formal methods usage in industries. Objective: We aim to evaluate the acceptance of formal methods by engineers if the complexity of understanding verification results is made easy. Method: We perform two different exploratory studies. First, we conduct an online survey to explore challenges in identifying inconsistent specifications and using formal methods from engineers. Second, we perform a one group pretest and posttest experiment to collect impressions from engineers using formal methods if understanding verification results is eased. Limitations: The main limitation of this study is the generalization because the survey focuses on a particular target group and it uses a pre-experimental design.

==> tex/responseletter.tex <==
\onecolumn
\noindent\add{We would like to thank the anonymous reviewers for their valuable comments, which helped us improve the manuscript. In the following, we do not address the positive feedback and focus only on the reviewers' questions. The following responses and according changes to the manuscript are highlighted in blue.}

\section*{Reviewer 1}
\noindent We thank the reviewer for the detailed comments and for highlighting the portions that need to be discussed explicitly. .
\vspace{7pt}

\noindent\textbf{R1.1)} The two parts of the study (corresponding to goals G1 and G2) are at quite different levels of generality. G1 is about challenges of identifying inconsistent specifications in a broader context, whereas G2 focuses on the understandability of model-checking counterexamples. The two levels are an effective way of organizing the research questions. However, the gap between the two levels remains fairly wide. Maybe you can think about adding a research question that explicitly connects the two levels. Perhaps this is already implicit in answering RQ1 and RQ2, but the design would benefit from a more explicit discussion of this aspect.
\vspace{3pt}

\noindent\add{Thanks for pointing at this gap. We rephrased RQ3 in the revised draft under the section \textit{Research Questions}.}
\vspace{3pt}

\noindent\add{RQ3: To what extent do engineers prefer to use formal methods (model checkers particularly) if the difficulty is reduced for understanding verification results to identify inconsistent specifications?}
\vspace{7pt}

\noindent\textbf{R1.2)} For Part 2, have you considered a different experimental design where a participant is assigned a different treatment (in this case, only the counterexample, or the counterexample plus the additional explanation) on different tasks, and the tasks are chosen to be sufficiently different (for example, they refer to different parts of the system)? This way, provided the risk of a learning effect can be reduced, there would be a more robust design. Perhaps this is not feasible in terms of required resources; but you could explicitly discuss it and give reasons for why it may or may not be infeasible.
\vspace{3pt}

\noindent\add{First, lets say that we are fully aware of the limitations of our design choice for our experimental design. As discussed in the subsection Part 2: One-Group Pretest-Posttest Design, one of the main drawbacks of using a one-group pretest-posttest design is that it does not meet the scientific standards of an experimental design. For example, the pre-experimental study designs do not have a control group like a true experiment. Thus, comparison and generalization of the results based on the provided intervention/stimulus may not be possible.}
\vspace{3pt}

\noindent\add{However our decision for a pre-experimental user study design is based on the scarcity of potential participants. To find a considerable number of participants (30 to 40) with knowledge of formal methods and model checkers inside an industrial organization is ambitious. Yet, performing a true experiment with a lower number of participants would raise the threat to the external validity of our study. Therefore, we intend to perform a one-group pretest-posttest experiment with Bosch automotive engineers that allow us to capture results from real-world user behavior with the limited number of potential participants.}
\vspace{7pt}

\noindent\textbf{R1.3)} Do you plan to do only visualization for the data in Part 2 of the study? Do you think statistics would not be justified given the limited number of participants? Here too, I think these points are worth discussing even if they would confirm my guess about the reasons behind them.
\vspace{3pt}

\noindent\add{In order to argue the results with statistics, we need two different groups of participants. With these two groups, it is possible to perform a true experiment to obtain the statistical analysis. However, since we follow a one-group pretest-posttest design due to the limited number of industrial participants, we would prefer to choose qualitative analysis and resort to descriptive statistics and visualisation to help the reader to understand our qualitative results.}
\vspace{7pt}

\noindent\textbf{R1.4)} Section III.A: I'm not sure I understand what the expression "add-on to system safety" is supposed to mean as a variable. Could you find a clearer expression (perhaps "increase in confidence in system safety/correctness"?)
\vspace{3pt}

\noindent\add{We revised the name of the variable according to the suggestion, i.e., “increase in confidence in system safety”.}
\vspace{7pt}

\section*{Reviewer 2}

\noindent We thank the reviewer for the detailed comments and for highlighting weak spots in our design. We agree with the reviewer’s comments and have already considered these points as threats as well as discussed to handle these threats in the \textit{Threats to Validity} section.
\vspace{7pt}

\noindent\textbf{R2.1)} To be honest, I find them a bit unambitious: Increasing preference is frail evidence. I could argue that any additional information might increase the subjective preference. Why do you avoid measuring any kind of actual improvement in understanding?
\vspace{3pt}

\noindent\add{In order to measure an actual improvement, a true experiment with a control group would need to be performed. However, due to the lack of a significantly large number Bosch engineers with formal methods expertise, we would not find enough participants to perform a true experiment. The pre-experimental design is therefore a compromise to yield assertive results with this limited number of participants. These results will help the field and provide a stepping stone for future investigations and experiments.}
%\vspace{3pt}

\noindent\add{We provide measures to mitigate potential threats to validity. The threat of history/maturation is mitigated to a certain degree by explicitly stating to participants that the study results will serve as a reference in the future to use our counterexample explanation approach for real-world projects at Bosch. Additionally, to avoid overwhelmed responses and accept only valid responses, we will cross-check the answers provided for the task questions (TQ1 to TQ9). Further, to reduce biasing between the pretest and the posttest experiment, the use case of an airbag system (a toy example) used in the pretest is significantly less complex than the use case of the Bosch EPS system.}
\vspace{7pt}

\noindent\textbf{R2.2)} In Tables I, II and III: Only LS6 is actually a Likert Scale. All the others are simply ordinal scales.
\vspace{3pt}

\noindent\add{Agreed, we use the Likert Scale and 7 point answer scales. As a result we changed the term now to Likert and answer scales.}
\vspace{7pt}

\noindent\textbf{R2.3)} I was wondering a bit why you need an entirely new questionnaire. What about reusing the TAM2?
\vspace{3pt}

\noindent\add{We agree with the reviewer’s suggestion of considering using the TAM2 model since part of the study also deals with usability. However, since we were able to adapt the structure of the pretest-posttest experiment and questionnaire from Zaidman et al.~[ZaidmanMSD13], we decided to reuse the same then using TAM2 model.}
\vspace{3pt}

\noindent\add{[ZaidmanMSD13] A. Zaidman, N. Matthijssen, M. D. Storey, and A. van Deursen, “Understanding ajax applications by connecting client and server-side execution traces,” Empir. Softw. Eng., vol. 18, no. 2, pp. 181–218, 2013.}
\vspace{7pt}

\noindent\textbf{R2.4)} I think one can argue for the pre-post-test design. Yet, I think a design with a control group comparing differences in understanding would be much stronger, even if the statistical power might be weak. I would rather argue that replications could ramify this. Instead, with your design, we only learn possible changes in preference that might be caused by other effects.
\vspace{3pt}

\noindent\add{We thank the reviewer for highlighting this option. During our early phase of design, we had the same opinion. However, considering the threats due to the limited number of participants for a controlled experiment (see response R1.2, R2.1), we believe threats listed by Campbell and Stanley [CampbellS63] for the one-group pretest-posttest experiment can be handled. We came to this conclusion also by considering Zaidman et al.~[ZaidmanMSD13] work as a reference.}
\vspace{3pt}

\noindent\add{[CampbellS63] D. T. Campbell and J. C. Stanley, Experimental and quasi-experimental designs for research. Rand McNally Chicago, 1963.}
\vspace{3pt}

\noindent\add{[ZaidmanMSD13] A. Zaidman, N. Matthijssen, M. D. Storey, and A. van Deursen, “Understanding ajax applications by connecting client and server-side execution traces,” Empir. Softw. Eng., vol. 18, no. 2, pp. 181–218, 2013.}
\vspace{7pt}

\section*{Reviewer 3}
\noindent We thank the reviewer for the comments and for highlighting the portions that need to be discussed explicitly.
\vspace{7pt}

\noindent\textbf{R3.1)} Some previous studies have identified challenges or difficulties in using formal methods to develop software systems. What is the special significance of this work designed for Bosch automotive engineers? Therefore, the authors should highlight the difference between this work and previous studies.
\vspace{3pt}

\noindent\add{The following details are added in the revised draft under the subsection \textit{Part 1: Online Survey}. We refer to and adapt some of the questionnaires from existing latest user surveys by Gleirscher and Marmsoler [GleirscherM20], and Garavel et al.~[GaravelBP20]. Gleirscher and Marmsoler [GleirscherM20] perform the largest cross sectional survey with 216 participants to study the existing and intended use of formal methods. Similarly, Garavel et al. [GaravelBP20] conduct a user survey with 130 participants and 30 questions to collect information on the past, present, and future of formal methods in research, industry, and education. The major differences our study makes to the existing surveys are: (1) most of the surveys focus on general challenges using formal methods, but we specifically focus on identifying challenges that engineers face in identifying inconsistent specifications as well as an understanding counterexample, and (2) the study is performed with the engineers who work on real-world projects.}
\vspace{3pt}

\noindent\add{[GleirscherM20] M. Gleirscher and D. Marmsoler, “Formal methods in dependable systems engineering: a survey of professionals from europe and north america,” Empir. Softw. Eng., vol. 25, no. 6, pp. 4473–4546, 2020.}
\vspace{3pt}

\noindent\add{[GaravelBP20] H. Garavel, M. H. ter Beek, and J. van de Pol, “The 2020 expert survey on formal methods,” in Formal Methods for Industrial Critical Systems -25th International Conference, FMICS 2020, pp. 3–69.}
\vspace{7pt}

\noindent\textbf{R3.2)} As the authors stated, Part 2 of this study is an exploratory pre-experimental user study. Why not design controlled experiments by offering a training course for selected engineers? The reviewer believes that this experiment may be more valuable to answer RQ3.
\vspace{3pt}

\noindent\add{We agree that a true experiment would be beneficial. The study design is a compromise due to the limited number of potential participants with formal methods expertise within Bosch, see responses to R2.1 and R2.4. Additionally, as a small side note the didactic skills of people of the training course and several other aspects will be confounding factors for the experiment that would limit the trustworthiness of a full controlled experiments. As a result we made this design choice.}
\vspace{7pt}

\noindent\textbf{R3.3)} In the reviewer's opinion, this work may output more qualitative analysis results. Why not use quantitative analysis methods?
\vspace{3pt}

\noindent\add{The qualitative results of the study study with engineers working on real-world projects will be valuable for the community to better understand the problem and its context. We decided against heavy use of quantitative analysis methods because of the nature of our experimental design.  %The primary threat with our user-study design is the limited number of participants. However, even with this limited number, we perform the study with engineers working on real-world projects.
However, we providing quantitative results collected from our engineers as much as possible to enrich the qualitative evaluation.}
\vspace{7pt}

\noindent\textbf{R3.4)} Do the authors plan to design and develop a formal verification-oriented translator for end engineers to facilitate the development process using formal methods? The reviewer believes that this work may make more sense.
\vspace{3pt}

\noindent\add{Absolutely! Modeling the system model and formalizing specifications are performed using the framework FASTEN~[RatiuNMCV21] for the counterexample explanation approach we discussed in Part 2. This framework has explicit and extensive support for domain-specific (or even project-specific) abstractions and visualizations. We started working on domain-specific explanations and will continue to do so.}
\vspace{3pt}

\noindent\add{[RatiuNMCV21] Ratiu D., Nordmann A., Munk P., Carlan C., Voelter M. (2021) FASTEN: An Extensible Platform to Experiment with Rigorous Modeling of Safety-Critical Systems. In: Domain-Specific Languages in Practice. Springer, Cham.}
\vspace{7pt}

\noindent\textbf{R3.5)} The apparent limitation of a specific domain (automobile) and a single company (Bosch).
\vspace{3pt}

\noindent\add{While the focus of our survey might look like a single domain and company, automotive is an important safety-critical domain, where complexity is rising. We argue that automotive is therefore a domain particularly suited to investigate our research questions. Additionally, Bosch is the world’s biggest automotive supplier.  Thus, we believe our study result will be valuable to the community to know the potential challenges using formal methods specifically on counterexample interpretation or identifying inconsistent specifications for safety-critical applications. }

\newpage
\twocolumn 
